Claim Extraction for Fact-Checking: Data, Models, and Automated Metrics

In this paper, we explore the problem of Claim Extraction using one-to-many text generation methods, comparing LLMs, small summarization models finetuned for the task, and a previous NER-centric baseline QACG. As the current publications on Claim Extraction, Fact Extraction, Claim Generation and Check-worthy Claim Detection are quite scattered in their means and terminology, we compile their common objectives, releasing the FEVERFact dataset, with 17K atomic factual claims extracted from 4K contextualised Wikipedia sentences, adapted from the original FEVER. We compile the known objectives into an Evaluation framework of: Atomicity, Fluency, Decontextualization, Faithfulness checked for each generated claim separately, and Focus and Coverage measured against the full set of predicted claims for a single input. For each metric, we implement a scale using a reduction to an already-explored NLP task. We validate our metrics against human grading of generic claims, to see that the model ranking on $F_{fact}$, our hardest metric, did not change and the evaluation framework approximates human grading very closely in terms of $F_1$ and RMSE.

==> changer.tex <==
\begin{table*}
    \centering

    \begin{tabular}{l|cccc|cccc}
        %\hline
        & \multicolumn{4}{c|}{\s{Automated Metrics}} & \multicolumn{4}{c}{\s{Gold Annotations}} \\
        {Model}                                           & $A$        & $G$      & $D$      & $Faith$ & $A_g$     & $G_g$    & $D_g$    & $F_g$    \\
        \hline           
        \footnotesize{\texttt{qacg}}                      & 0.89       & 0.69     & 0.70     & 0.88    & 0.99      & 0.85     & 0.91     & 0.76     \\
        \footnotesize{\texttt{gpt-4-turbo-3-shot}}        & 0.92       & 0.70     & 0.77     & \s{0.99}& 0.98      & \s{0.97} & \s{0.96} & \s{0.93} \\
        \footnotesize{\texttt{qlora-mistral-instruct}}    & 0.95       & 0.75     & 0.80     & 0.95    & \s{1.00}  & 0.96     & \s{0.96} & 0.90     \\
        \footnotesize{\texttt{t5\_sm\_diverse\_7\_beams}} & 0.95       & 0.74     & 0.80     & 0.91    & 0.99      & 0.89     & 0.95     & 0.79     \\
        \footnotesize{\texttt{t5\_sm\_multi-claim}}       & \s{0.96}   & \s{0.76} & \s{0.82} & 0.95    & \s{1.00}  & 0.91     & 0.94     & 0.88     \\
        \hline
    \end{tabular}
    \caption{\label{model-comparison-bin}
        Model comparison on means of model metrics over all samples (or over all annotated samples). In bold are the best values for each metric.}
\end{table*}

==> src/related.tex <==
%!TEX ROOT=../acl2023.tex
\section{Related work}\label{sec:related}

\begin{enumerate}
    \item \textbf{XSum}~\cite{narayan-etal-2018-dont} -- single sentence summaries on a large scale -- match the claim structure very close, except for atomicity.
    \item \textbf{FEVER}~\cite{fever-2022-fact,thorne-vlachos-2021-evidence} -- recently republished along with Wikipedia abstracts that were used to extract claims -- may be a great testbed for our specific summarization task.
    \item \textbf{CLEF CheckThat}~\cite{barroncedeno2020overview} -- series of shared task that published numerous datasets on the adjacent task of checkworthiness estimation and evaluation schemes for the solution, also, generating claims from social media
    \item \textbf{BERTScore}~\cite{bert-score} proposes a precision, recall and F1 score for the seq2seq tasks based on the BERT-model embeddings
    \item \textbf{FFCI}~\cite{ffci} takes these scores to estimate \textit{faithfulness}, \textit{coverage}, \textit{focus}, \textit{coherence} and other scores typical for abstractive summarization
    \item \textbf{Scientific Claim Generation}~\cite{wright-etal-2022-generating} gives a functioning scheme of transducing source \textit{citances}\footnote{Self-contained (citable) factual sentence.} to atomic claims -- this could either be used for comparison, or later in our pipeline to \q{atomize} our extracted claims, as those have a form of a citance.
    \item \textbf{QAGS}~\cite{wang-etal-2020-asking} gives methods for examining claim \textit{focus} and \textit{coverage} using QA methods, and proposes a method for extracting claims from source texts using NERs and QA
    \item \textbf{AlignSCORE}~\cite{zha-etal-2023-alignscore} proposes a method for checking factual consistency of various text2text tasks using a function aligning factual information in two arbitrary texts
    \item \todo{More recent works in field? (the above was updated in April)}
\end{enumerate}


